Why Synchronized Time is a Fiction: Daylight Saving Time, Leap Seconds, and the Guillotine Sharpened for Nothing

Civilization maintains an elaborate infrastructure devoted to the maintenance of synchronized time. Governments mandate daylight saving time. Standards bodies insert leap seconds into Coordinated Universal Time. Engineers debate leap milliseconds and leap nanoseconds. The Global Positioning System applies relativistic corrections at the nanosecond level. All of these adjustments attempt to preserve an assumption: that a single global time exists and that clocks can be made to agree upon it. This paper argues that this assumption constitutes a category mistake in the sense of Ryle (1949). We show that special and general relativity prohibit absolute simultaneity, that the one-way speed of light is conventionally defined rather than measured, and that recent experiments on indefinite causal order demonstrate nature admits correlations with no well-defined temporal sequence. We trace the consequences of this category mistake through distributed computing, where it manifests as the Forward-In-Time-Only (FITO) assumption that underlies Lamport's logical clocks (1978), the impossibility results of Fischer-Lynch-Paterson (1985), and the CAP theorem (2000). From this perspective, daylight saving time and leap seconds are not corrections to time but corrections to conventions -- they sharpen the guillotine of synchronization in preparation for executing something that does not exist.

==> dae-handout-commands.tex <==
% --- dae_commands.tex ---

% --- FAQ/Answer macros ---
\newcommand{\question}[1]{%
  \stepcounter{qctr}%
  \vspace{5pt}
  \noindent
  \rule{0.5\columnwidth}{0.5pt}\\
  \noindent
  \phantomsection
  \textbf{[Q\decimal{qctr}]}~%
  \def\a##1\par{##1}{#1}%
  \addcontentsline{loq}{section}{Q\protect\numberline{\theqctr}{{#1}}}
}

\newcommand{\answer}{%
  \vspace{5pt}
  \noindent
  \textbf{[A\decimal{qctr}]}
}

\newcommand{\statement}{%
  \vspace{5pt}
  \noindent
  \textbf{[S\decimal{qctr}] Statement: }
}

\newcommand{\insight}{%
  \vspace{5pt}
  \noindent
  \textbf{[A\decimal{qctr}} Insight: ]
}

\newcommand{\sublistofquestions}{%
  \onlyinsubfile{\vspace{0pt} \large \listofquestions \normalsize \medskip}
}

% --- Subfiles helpers ---
\newcommand{\onlyinsubfile}[1]{#1}
\newcommand{\notinsubfile}[1]{}

% --- Insert Hyperlink (file) ---
\newcommand{\ihl}[2]{%
  \vspace{6pt} \noindent [\hyperlink{./Exhibits/#1.pdf.1}{#1}]{ #2}
}

% --- Insert Menu Item (file/comment) ---
\newcommand{\imi}[2]{%
  \vspace{10pt}
  \noindent
  \textbf{\href{run:FAQ-#1.pdf}{#1}}\\{#2}
}

% --- Strikeout Displaystyle ---
\newcommand{\displayst}[1]{\textrm{\st{$\displaystyle#1$}}}

% --- Custom Horizontal Rule ---
\newcommand{\srule}{%
  \vspace{2pt}
  \noindent\rule{\textwidth}{0.8pt}
}

% --- Leibniz Bridge sibling document references ─────────────────
% \daeref{label}{filename}{description}
%   Links to a sibling document in the same project folder.
%   Rendered in linkred. Margin note shows label + description.
%   Auto-detects format from extension and annotates [PDF] or [HTML].
%   Uses \href{run:filename} so macOS opens the right application.
%   In arXiv/HTML mode: becomes a footnote (no margin note).
%
% Usage:
%   \daeref{DAE-TR-0007}{DAE-TR-0007.pdf}{The Category Mistake}
%   \daeref{CAP Paper}{oae-cap-tufte.html}{HTML with responsive sidenotes}
%
\makeatletter
\newcommand{\dae@detectformat}[1]{%
  \dae@checkhtml#1.html\@nil
}
\def\dae@checkhtml#1.html#2\@nil{%
  \def\dae@temp{#2}%
  \ifx\dae@temp\empty
    \def\dae@fmt{PDF}%  no .html found, assume PDF
  \else
    \def\dae@fmt{HTML}%
  \fi
}
\ifarxiv
  \newcommand{\daeref}[3]{%
    \dae@detectformat{#2}%
    \href{#2}{\textcolor{linkred}{#1}}%
    \footnote{\textcolor{linkred}{#1}\enspace[\dae@fmt]\enspace #3}%
  }
\else
  \newcommand{\daeref}[3]{%
    \dae@detectformat{#2}%
    \href{run:#2}{\textcolor{linkred}{#1}}%
    \marginnote{\scriptsize\textcolor{linkred}{#1}\enspace\textsc{[\dae@fmt]}:\enspace #3}%
  }
\fi
\makeatother

% --- Leibniz Bridge Margin TOC (standardized) ---
% Usage: place \daemargintoc after \maketitle / \placebadges on the first page.
% Requires: etoc, hyperref, linkgreen colour defined,
%           Bitstream Charter via mathdesign (provides bold small caps).
% Sections: bold small caps, green, with number.
% Subsections: regular small caps, green, indented.
% Section short titles MUST be in Title Case for the small-caps effect.
% In arXiv/HTML mode: suppressed (arXiv generates its own TOC sidebar).
\newcommand{\daemargintoc}{%
  \ifarxiv\else
  \marginnote{%
    \hypersetup{linkcolor=linkgreen}%
    \small
    \setcounter{tocdepth}{2}%
    \etocsetstyle{section}{}{\par\vspace{1em}\noindent\leftskip=0em%
      \parbox[c]{1.5em}{\centering\etocnumber}%
      \parbox[c]{\dimexpr\marginparwidth-3em\relax}{\linespread{0.75}\selectfont\raggedright\textbf{\textsc{\etocname}}}%
      \hfill\etocpage\par}{}{}%
    \etocsetstyle{subsection}{}{\par\vspace{0.5em}\noindent\leftskip=1.5em%
      \parbox[c]{1.5em}{\centering\etocnumber}%
      \parbox[c]{\dimexpr\marginparwidth-3em\relax}{\linespread{0.75}\selectfont\raggedright\textsc{\etocname}}%
      \hfill\etocpage\par}{}{}%
    \etocsettocstyle{}{}%
    \tableofcontents
  }%
  \fi
}

\NewDocumentCommand{\marginfig}{O{width=\linewidth} m o o o o}{%
  \begin{marginfigure}\IfValueT{#6}{[#6]}%
    \IfValueTF{#5}{#5}{\centering}%
    \includegraphics[#1]{#2}%
    \IfValueTF{#3}{%
      \caption{#3}%
    }{%
      \caption{#2}%
    }
    \IfValueTF{#4}{%
      \label{#4}%
    }{%
      \label{fig:#2}%
    }
  \end{marginfigure}
}

\NewDocumentCommand{\fig}{O{width=\linewidth} m o o}{%
  \begin{figure}
    \centering
    \includegraphics[#1]{#2}% 
    \IfValueTF{#3}{%
      \caption{#3}%
    }{%
      \caption{#2}%
    }
    \IfValueTF{#4}{%
      \label{#4}%
    }{%
      \label{fig:#2}%
    }
  \end{figure}
}


==> dae-handout-settings.tex <==
% Document class

% Core packages
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{microtype}
\usepackage{xparse}
\usepackage{amsmath,amssymb}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{lipsum}
\usepackage{epigraph}
\usepackage{framed}
\usepackage{todonotes}
\usepackage[most]{tcolorbox}

% Specialized
\usepackage{tikz}
% \usepackage{bytefield}  % DEPRECATED (2026-03-10) — not available in all TeX Live installations
\usepackage{eso-pic}

% Graphics path (Leibniz Bridge convention):
%   ./figures/    — local working copies (populated by pull-figures.sh)
%   ../Figures/   — shared parent folder
%   ../../Figures/ — grandparent
%   FIGURES/      — absolute iCloud master (last resort)
\graphicspath{{./}{./figures/}{../Figures/}{../../Figures/}{./images/}{./graphics/}}

% ── Leibniz Bridge colour scheme ─────────────────────────────────
% Green: internal navigation (same document) — \ref, \cite, TOC
% Blue:  external web links — \url, \href to http(s)
% Red:   sibling documents (PDF, HTML in same project folder)
\definecolor{linkblue}{RGB}{30, 80, 180}
\definecolor{linkgreen}{RGB}{30, 120, 60}
\definecolor{linkred}{HTML}{AE0000}

% Hyperref
\usepackage{hyperref}
\hypersetup{
  colorlinks=true,
  urlcolor=linkblue,          % \url and \href to web
  linkcolor=linkgreen,        % \ref, \eqref, \pageref, TOC
  citecolor=linkgreen,        % \cite (jumps to bib within this doc)
  filecolor=linkred,          % \href{run:...} local file links
}

% Font commands
\newcommand{\headerfont}{\fontfamily{phv}\selectfont}
\newcommand{\titlefont}{\headerfont\Huge\bfseries}
\newcommand{\authorfont}{\headerfont\large}
\newcommand{\datefont}{\headerfont\normalsize}

% Custom title page
\makeatletter
\renewcommand{\maketitle}{
  \newpage
  \thispagestyle{empty}
  \begin{fullwidth}
    \centering
    {\titlefont \@title \par}
    \vspace{1em}
    \ifx\@author\@empty\else
      {\authorfont \@author \par}
      \vspace{0.5em}
    \fi
    \ifx\@date\@empty\else
      {\datefont \@date \par}
    \fi
    \vspace{2em}
  \end{fullwidth}
}
\makeatother

% Custom abstract
\newenvironment{customabstract}{
  \begin{fullwidth}
  \begin{adjustwidth}{0.5in}{0.5in}
  \vspace{1em}
  \small
  \color{gray!30!black}
}{
  \vspace{1.5em}
  \end{adjustwidth}
  \end{fullwidth}
}



% Unicode fallback
\DeclareUnicodeCharacter{2E3B}{\textbar\textbar}

% Optional: comment out subfiles you're not using
%\includeonly{Protocol-Byte-Content}

